How Much is Performance Worth to Users? A Quantitative Approach

Architects and systems designers artfully balance multiple competing design constraints during the design process but are unable to translate between system metrics and end user experience. This work presents three methodologies to fill in this gap. The first is an incentive-compatible methodology that determines a "ground truth" measurement of users' value of speed in terms of US dollars, and find that users would accept a performance losses of 10%, 20%, and 30% to their personal computer in exchange for \$2.27, \$4.07, and \$4.43 per day, respectively. However, while highly accurate the methodology is a painstaking process and does not scale with large numbers of participants. To allow for scalability, we introduce a second methodology -- a lab-based simulation experiment -- which finds that users would accept a permanent performance loss of 10%, 20%, and 30% to their personal computer in exchange for \$127, \$169, and \$823, respectively. Finally, to allow for even greater scalability, we introduce a third methodology -- a survey -- and observe that the lack of incentive compatibility and the lack of hands-on experience with throttled device performance skews the results significantly, thus demonstrating the need for lab-based or incentive compatible study designs. By quantifying the tradeoff between user satisfaction and performance, we enable architects and systems designers to make more nuanced tradeoffs between design requirements.

==> background.tex <==
\section{Background} \label{sec:background}

The idea of pricing performance losses is not without precedent.
In recent years, several class action lawsuits have won large settlements from Apple for the so-called ``Batterygate'' scandal.
These lawsuits stemmed from allegations in 2017 that Apple had been deliberately slowing down older iPhones without the knowledge or consent of users \cite{batterygate}\footnote{Apple claimed this was done to mitigate the effects of aging batteries and to manage device temperature \cite{batterygate_response}, but it was rumored that Apple's ulterior motive was to degrade the performance of older iPhones to incentivize  owners to buy new iPhones.}.
In 2020, a U.S. district court in California approved a settlement of \$310--\$500 million, with an expected payout of \$25 per affected device~\cite{apple_ruling}.


The \$25 payout was agreed upon by both parties after the plaintiffs' damages consultant estimated a minimum damage of \$18 and a maximum damage of \$48 per device.
Court documents reveal that this \$18--\$48 estimation was based on the value of eligible devices in the secondary marketplace before and after the Batterygate disclosures \cite{apple_payouts}.

% Tie this to HW patches
This flat-rate payout based on available market data is a reasonable first-order approximation of the harms that users endured as a result of the performance-throttling updates. 
However, market prices alone may not reflect the true cost of performance throttling, and with the emergence of recent hardware vulnerabilities and their deleterious patches, the question of how to compensate users for performance losses may need to be examined from other angles.


\subsection{Hardware Patches}

Pricing the value of lost performance becomes especially important in the emerging era of hardware patches.
Unlike software patches, which typically come at little or no cost to performance, hardware patches often must take drastic measures to restore security and can greatly reducing system performance.
For example, the only surefire ``solution'' to the Spectre vulnerability is to disable speculative execution, which can hurt performance by up to 30--50\%\cite{kocher2019spectre, yu2019speculative}.
Additionally, practical Rowhammer defenses are not yet widely available \cite{trrespass}, and the only surefire defense is to drastically increase the DRAM refresh rate, dramatically decreasing system performance and dramatically increasing total energy consumption \cite{rowhammer}.
Other recent hardware patches can cause similar performance losses, and the many hardware vulnerabilities yet to be found will likely cause performance losses as well.






% The Batterygate lawsuits may be the first to demand payouts for performance losses but will likely not be the last.
% Recent 

% Patching security vulnerabilities in 

% An emerging precedent is beginning to take hold in the hardware industry:
% Hardware security issues are being discovered and patched after the product has shipped, much like the way software is fixed and patched.
% Although fixing security vulnerabilities is preferable to \textit{not} fixing them, the software patching model does not neatly extend to hardware, unfortunately. 
% This is because software patches and updates generally do not cause issues with system availability or performance.
% For example, memory safety bugs (which account for the majority of software vulnerability exploits found in the wild) can often be fixed with a simple adjustments such as by adding an array bounds check or by nullifying a pointer after it is freed.
% Such protections typically have a very small constant time overhead and generally have a negligible impact on overall system performance.

% In contrast hardware products are more or less immutable once they have been shipped, and when hardware vulnerabilities are found, they cannot be fixed by editing a few lines of code.
% The fixes must often take drastic measures to restore security.
% This has been seen with recent high-profile security vulnerabilities such as Spectre \cite{kocher2019spectre}.
% The official ``solutions'' to the vulnerabilities have been costly:
% For Spectre, the only surefire defense is disabling speculative execution, which can hurt performance by up to 30--50\%\cite{yu2019speculative}.
% Additionally, practical Rowhammer defenses are not yet widely available \cite{TRRespass}, and the only surefire defense is to drastically increase the DRAM refresh rate, dramatically decreasing system performance and dramatically increasing total energy consumption \cite{Rowhammer}.
% Other recent hardware patches can cause similar performance losses, and the many hardware vulnerabilities yet to be found will likely cause performance losses as well.

% For this reason alone, we cannot accept the nascent practice of hardware patches to be administered in the same way we handle software patches.
% It is unfair to consumers, who buy products with the expectation that they are reasonably secure, only to later find that they must accept performance losses to achieve the level of security they had assumed when purchasing the product.
% With more hardware vulnerabilities likely waiting to be discovered, and with more performance-degrading patches yet to be issued, it is of high importance that the precedent of software patching does not take root in the hardware community.



% \subsection{Willingness to Accept}

% One such angle proposed in this work is measuring users' willingness to accept performance losses in their personal devices. 
% A ``willingness to accept'' (WTA) is the lowest monetary amount a person or entity would be willing to accept in exchange for some unfavorable condition or outcome.
% % In this work, we aim to find participants' willingness to accept a slowdown to their computer's performance.
% % We seek to find this number since it demonstrates how much users who voluntarily apply performance-sapping hardware patches are willing to pay to remain secure. 

% Finding users' willingness to accept various degrees of performance losses can inform us on the harms done to users by performance-throttling patches and updates, but also indirectly informs us on users willingness to \textit{pay} for security, in terms of performance.
% For example, if a user would require a minimum of $\$X$ to accept a device slowdown of $Y\%$, and if this user would voluntarily apply a security patch that reduces performance by $Y\%$ in an effort to remain secure, then is is implied that the user values the security offered by the patch at least $\$X$.

% % If the goal is to find out how much users value security, why find the willingness to accept performance losses and not the willingness to accept security losses?
% % The answer is that designing incentive-compatible experiments that ask participants to forgo security in exchange for money exposes participants to a non-negligible level of risk and would cross guidelines of ethical human subjects research.
% % Therefore, we must rely on the value of performance to act as a proxy for the value of security.

% % The second question our experiments aim to answer is how much performance can be ``consumed'' by security features before the slowdowns are noticeable to users.
% % The benefit of answering this question is that it informs us on users' tolerance for performance-throttling patches.
% % For example, if a patch slows down performance by $Y\%$, but we find that a $Y\%$ slowdown causes only an imperceptible difference for the average users' experience, then we can conclude that such patches are tolerable and may be worth the slowdown if they improve security in a meaningful way.

% % \subsection{Externalized Insecurity}

% % TODO:

% % This section is on why this data is important in an area with little to no regulation. 

% % We don't want hardware companies to be able to externalize their security failures onto customers after the products have already been purchased.

% % Market failures mean that this area is not going to fix itself without regulation;
% % Regulation and policy is going to fail if it is unifmored on the value of the performance lost


==> fw.tex <==
\section{Future Work}
\label{sec:fw}

% This is just a starting point
% In the search of quantifying the price of security, there is a large space of experiments that can be conducted.
% The studies presented in this paper are only the starting point in a series of many experiments 
% In this section, we discuss possible variants of the experiment we conducted as well as other study designs we considered that can help answer adjacent questions.

An indicator of good research paper is that it raises more questions
than it answers.  The experiments presented in this paper are only
two of many experiments we considered running.  These two experiments
represent a starting point for research in an area that is at the
intersection of hardware security, user behavior and economics.  As
such, there is a huge space for further experimentation.  In this
section, we discuss some potential directions.

% Running Experiment 1 but informing participants of slowdowns.
% Just because you don't know you're being poisoned doesn't make it OK!
% An obvious candidate for future work is to repeat Experiment \#1 but with first informing pariticipants that their device will be throttled during one of the three sets of tasks.
% This 

\comment{
An obvious candidate for future work is to repeat Experiment \#1 but without the deception (recall that while completing the tasks, participants in Experiment \#1 were unaware that their computer's speed was at times being throttled).
We found the deception to be necessary to answer the specific questions we were after;
however, disclosing the performance slowdowns to participants \textit{before} they complete the tasks can help answer a different set of questions altogether.
For example, it would be interesting to find out how perceptive study participants are to performance slowdowns when they are explicitly told that their computer's speed may be throttled during some of the tasks.
Such participants would almost certainly be more perceptive to noticing the slowdowns, but by how much?
If the margins are small, does this justify imposing performance-throttling security patches without users' consent, since it would confirm that performance slowdowns do not significantly affect the user experience?
% And if the margins are large, does this imply that 


Another possible variant of Experiment \#1 is to not only inform participants that their device may be slowed down at some point but to explicitly inform during \textit{which task} their device is running slower.
This protocol does not answer any questions regarding users' perceptiveness of slowdowns but may help participants make better informed decisions when deciding their willingness to accept performance slowdowns, since participants can consciously take note of the effects of a slowdown when completing the tasks.
We note that such a protocol still lacks incentive compatibility, and that participants are free to reply with any answer without consequence.



% Why did we decide to deceive?

% Running Protocol 2 at more slowdowns

Another obvious candidate for future work is to repeat Experiment \#2 at additional slowdown percentages.
Our own experiments only tested participants' willingness to accept a patch that throttles performance by 30\%, since this matches slowdowns seen by some recent hardware patches, but the experiment can be repeated for any slowdown percentage.
If repeated across enough slowdown percentages, one could plot the demand curve for performance in terms of daily WTA price.
This data would be valuable to vendors and regulators, who are both new to the nascent practice of issuing rebates for performance throttling patches and updates (this is discussed more in Section~\ref{sec:takeaways}).
The main hindrance to running such experiments is that their incentive-compatible nature makes them much more expensive to run.

%Titration wrt performance---at what point do they break?
% In addition to extending the experiments presented in this paper, other 
Experiment \#2 can be conducted in reverse: rather than giving participants a range of different offer prices for a fixed-percentage slowdown, one could instead offer a range of different slowdown percentages for a fixed payout amount. 
This answers the complementary question of ``how much performance are users willing to forgo in exchange for $\$X$?''
Again, by running such an experiment across a range of different payout prices, one could use regression techniques to determine the general relationship between performance lost and willingness to accept.

%titration
Further variations include titration-like protocols, where the degree of slowdown imposed on participants' devices is slowly increased (or alternatively, the amount of money offered per day slowly decreased) until the participant reaches a ``breaking point'' at which the offer money is no longer worth the slowdown imposed on their device.
Like our Experiment \#2, this protocol also finds an incentive compatible answer to the question of how much users value their devices' performance.



% Other variants and experiments discussed but not implemented
In addition to running variants of the two experiments in this paper, different experimental protocols altogether can  help answer additional and adjacent questions.
For example, consider a study that profiles user behavior before and after a performance-throttling patch.
Does a loss of performance increase the amount of time it takes users to perform everyday tasks?
Does a loss of performance cause users to experience more frustration when using their device?
Does it cause them to use their device less?
Answering these questions helps us quantify the costs that users must pay when accepting security patches and updates.


% Profiling. But we don't know how to interpret the data.

}


==> motivation.tex <==
\section{Payout Models} \label{sec:motivation}

We briefly discuss the various models that available for determining how much is owed to consumers whose products are degraded after purchase.

\subsection{Flat Rate Payouts}

The simplest method of compensation is to pay a flat rate to all consumers who were financially harmed via patches.
This is the approach taken in \textit{Naylor et al v. Apple}, where each injured party could claim \$25 for a maximum settlement of \$500 million.
In \textit{Naylor et al. v. Apple}, it was not publicly revealed how this flat rate was reached.
In a world with little established precedent, an absence of pertinent data, and a lack of more technical or sophisticated solutions, we expect that that the flat rate payout model will become the dominant payout method.

We discuss two methods of determining a flat-rate payout.

\subsubsection{Resale value}
The first option is to pay injured parties the amount of resale value lost due to the patch.
The formula is as follows:
First, the resale price $\$p$ of the consumer's product \textit{before} the performance-throttling patch is determined by looking at the prices of similar products with the same performance level pre-patch.
After the patch is applied, the product becomes less valuable and will sell at the new resale price $\$q$.
% Need to explain that product is less valuable even though it is more secure.
% This is because the assumed security level remains constant throughout (both pre- and post-patch)
A fair compensation would then be $p - q$, or the difference in value of the product pre- and post-patch.
This model is fair because a consumer who really needs the pre-patch levels of performance can sell their current device for $\$q$ and combine the profit with their $\$p - \$q$ rebate to get $\$q + \$p - \$q = \$p$ and purchase a product with performance comparable to their pre-patch device.
Likewise, a consumer who doesn't need that extra performance can pocket the $p - q$.

% Some problems exist with the flat rate payout approach:

% Problems:
% Sometimes monopolies make it hard to find comparable devices
% Hard to replace device
% 

\subsubsection{Harm-based payouts}
An alternate method is to find a dollar equivalent of the harm done to consumers as a result of the patch.
One possible approach is to find the willingness of consumers to accept the slowdown resulting from the patch in terms of dollars.
For example, if the average consumer would only accept a patch that throttles performance by 30\$ for no less than \$100, then the payout to the consumers should be \$100.
This work presents two methods for finding the price of people's willingness to accept such patches.

A significant issue with flat rate payouts is that not everyone will be affected the same way by such patches, and thus the payouts may be unfairly distributed (even if uniform).
For example, a cloud services company may suffer greatly from such patches if they have to compensate their loss of performance by purchasing additional servers.
On the other hand, a company who uses their systems only to store rarely-accessed databases may suffer no losses at all from a performance-throttling patch.
If the flat rate payout is set to the worst-case harm across all consumers, this might put hardware companies in financial ruin, which could stifle technological innovation.


% Complicating the matter is that it is very difficult to determine how to compare the two...
% Even companies that only use 
% Worker productivity?
% 


\subsection{Per-Case Payouts}

Perhaps a more equitable payout model would be to pay consumers on a case-by-case basis, where those who suffer more from a performance-throttling patch are compensated more for their troubles than those who do not suffer much at all.
We discuss two possibilities:

\subsubsection{Pay-as-you-go}
If the trend of performance-throttling patches becomes a commonplace occurrence, it might make sense to augment computer hardware with monitoring capabilities to determine the cumulative performance loss due to patches and issue recurring payouts to customers for the suffered performance losses.
% Would follow decreasing curve
This could rely on existing hardware performance counters in most CPUs or could require additional instrumentation to find fine-grained losses in performance.
The model would need to be tuned in such a way that caps the maximum payout to some set amount, or else consumers could, in bad faith, run continuous useless computations as a means to earn such pay-as-you-go rebates.


\subsubsection{Per-case harm-based payouts}
The pay-as-you-go approach would likely require tremendous changes to the hardware industry, and would likely be met with great resistance.
Perhaps there is an easier way to determine appropriate per-case payouts to the injured parties.
If there were a mechanism to find the approximate per-case harm caused by performance-throttling patches, perhaps per-case payouts could be achieved without requiring significant changes to existing hardware.
As with the flat-rate harm-based payouts, we could use willingness to accept such patches as the basis for such payouts, but consider them on a case-by-case basis rather than a flat rate computed from the averaged willingness to accept price.
The obvious issue is that there would be a tremendous incentive for companies and individuals to lie about how much harm they suffer from such patches.
Any such per-case harm-based payouts would need to be designed in such a way that incentivizes customers from reporting the true level of harm caused by losses in performance.
Such an incentive-compatible method is described in Section \ref{sec:methods}.

% How to not lie about WTA?


%\subsubsection{Liability}

% \subsection{Dynamic Payouts}

% \subsubsection{Pay-as-you-go}

% \subsection{Mechanism of Payout}

% \subsubsection{Per-case harm}

% \subsubsection{Class action lawsuits}




% Why we need companies to payout for slowing down their products

%\subsection{Problem Statement}

% Why would a company slow down their product? Two reasons...



% Incentive not to release patches?

% How can we make this INCENTIVE COMPATIBLE TODO!!!!


% Hardware is more immutable

% Fast mode vs safe mode? Not a good idea!

% A problem facing technology users today is that companies are free to degrade the quality or performance of their product in the field and without recourse.
% We examine two scenarios where a company may degrade performance of a product after it has been purchased.

% \subsubsection{Nefarious Updates}

% In 2017, it was discovered that Apple was quietly throttling the performance of older iPhones via software updates without users' knowledge or permission \cite{}.
% Only once the discovery was made did Apple admit to slowing down older iPhones as a way to mitigate effects of aging batteries and manage device temperature \cite{}.
% It was rumored the real purpose of the updates was to frustrate users of older iPhones and make them think their devices were slower and more out of date then they actually were, in an attempt to incentive the users into purchasing newer iPhone models. 

% % May be true

% % Recent class action lawsuit
% A class action lawsuit was filed against Apple in early 2018 over the allegations. 
% Two and a half years later, the Apple and the plaintiffs reached a settlement worth up to \$500 million with an anticipated payout of \$25 to each of the affected users.
% However, despite this very recent development, there are still no laws against such practices.
% It is likely that companies wishing to employ such practices in the future will find clever ways to slow down old devices while skirting the law.


% \subsubsection{Patch Embargoes and Externalized Insecurity}

% A counterintuitive aspect of hardware security is that it is sometimes rational for companies to \textit{not} fix outstanding security problems, or at least to delay disclosing the issue and releasing the patch for as long as possible.
% To explain this, consider the scenario where a team of researchers discover a hardware vulnerability in some product and notify the product vendor, in compliance with well-established vulnerability disclosure practices.
% Once the company is aware of the problem, the start to work on a patch but realize that the fix necessarily comes at the cost of performance.
% If the company issues the patch right away, the out-of-the-box performance of the device will decrease, and the product will be less competitive in the marketplace, costing the company sales and money. 
% However, if the company keeps the vulnerability hidden, then the unknowing public will continue to buy the product. 
% It is then in the company's rational self-interest to \textit{not} release the patch, or at least delay disclosure for as long as possible.
% The company's incentives are therefore at odds with the public's security.

% Some recent examples illustrate this principle in real-life.
% The MDS vulnerabilities found in some Intel processors were disclosed to Intel nearly a year before the vulnerabilities were publicly disclosed.
% % Likewise, Metldown was known for six months before a patch was released.

% % \subsection{Externalized Insecurity}



% % \subsection{Fast Mode vs. Secure Mode}


% % degrading devices after they're purchased

% % Externalizing insecurity

% % long patch period embargoes

% % An orthogonal issue is that 




% % So how do we deal with it?
% \subsection{Payout Models}

% Once we establish that device vendors should compensate customers for performance losses, the natural question to ask is how exactly this compensation should occur.
% We present and discuss three options an Authority could choose to enforce compensation. 

% \subsubsection{Device Replacement or Full Refund}

% The first and most drastic option is for the device vendors to issue a total recall of all affected products. 
% The argument is that the because the patch or update degrades performance, the product the consumers purchased is not the product the consumers received.
% In some cases, it may be that the customer demanded only the highest performance, and so the patch makes the customer's equipment worthless for their intended application. 
% Therefore, an interpretation of justice says that vendors should compensate their customers for the full price of the equipment.
% % Full refund from original price?
% % Full refund from depreciation price?
% This refund could be based on the original purchase price of the equipment, or possibly on the purchase price minus standard depreciation. 
% Alternatively, a vendor could offer a full replacement of the faulty product with a similar product of equivalent performance, pre-patch.

% % Too burdensome
% The issue with the full refund or replacement model is that it is prohibitively expensive for the vendors.
% A single vulnerability might be all it takes to bankrupt an entire company.
% The result would be that companies would be afraid to release any products at all, and the pace of technology would be slowed down, which is undesirable.
% % Not like prodcut safety recall, cause the patch ostensibly makes the product safe again
% Since we should expect that vulnerabilities will continue to be introduced into products in the future, we need a way to fairly compensate customers for slowdown patches without causing technology to grind to a halt.


% \subsubsection{Flat Rate Payouts}

% Another interpretation of justice says that companies should refund their customers with a partial rebate equivalent to the financial cost of a slowdown patch.
% % A vendor could also issue a partial rebate equivalent to the diminished value 
% There are two ways to do this:
% % First, the financial cost of a patch can be evaluated as the drop in market value before and after the patch. 
% First, the financial cost of a patch can be evaluated as the diminished value of a product as a result of the patch.
% We can use market resale price as a proxy for diminished value.
% For example, if some company's product sold for price $\$X$ before a patch but now only sells for price $\$Y$ (with $X > Y$), then  $X - Y$ is the loss of value each customer experienced as a result of the patch. 
% A company could issue this amount as a flat rate rebate to all customers to compensate them for their losses.

% Alternatively, a company could issue a flat rate rebate based on how much each customer would have to spend to regain the performance of the original product pre-patch. 
% For example, if a product of price $X$ and performance $A$ drops to market price $Y$ and performance $B$ after a patch (with $X > Y$ and $A > B$), and there remain a substitute product with price $Z$ and performance $A$, then the flat rate rebate issued to all customers should be $Z - Y$, so that consumers have the option to sell their degraded product for price $Y$ and use their cash $(Y)+(Z-Y) = Z$ to buy the substitute product at price $Z$ and regain the performance level $A$ the customers had originally intended to receive.

% % A permanent, irreversible, and performance-sapping patch can cause a financial loss to a vendor's customers because it decreases the product's economic utility and hence its value. 
% % Hence f

% % Market price?
% % Or cost to get customers to original service level?


% % How to calculate diminished value?
% % Market price before and after

% % Might sink a company

% % Resale value

% \subsubsection{Pay-as-you-go}

% A third option is pay-as-you-go.
% This model says that the amount a customer should be compensated for a patch should be equivalent to how much the customer has had to suffer as a result of the patch.
% As the name suggests, this is a per-case model, meaning that different customers may receive different payouts based on how much the patch affects them. 

% To illustrate an example, consider two users of a product, Alice and Bob.
% Alice uses applications that utilize the device's advanced performance-enhancing features, whereas Bob's applications only ever use the most basic features of the device.
% One day a security vulnerability is found in some of the device's advanced features, and so the device vendor issues a patch that disables these performance-enhancing features.
% % Alice is strongly affected by this patch whereas Bob is not affected at all.
% In the pay-as-you-go model, Bob does not need to be compensated for the patch, because he is not affected at all by the patch and suffers no losses from it.
% However, Alice deserves compensation, because the performance of her applications is significantly degraded.
% The pay-as-you-go model compensates Alice a small amount every time she is denied the performance she had originally purchased.
% We discuss how to price the value of this payout in Section \ref{}.

% The pay-as-you-go model is beneficial to both Alice and Bob because they are each compensated for the losses they have accrued as a result of the patch. 
% Likewise, if Bob starts using a new software tool that would have taken advantage of the advanced performance-enhancing features had they been available to use, Bob will also be compensated for accrued losses. 
% Thus this balances the need for companies to refund their customers on-demand, and without having to issue massive upfront costs to all users.


% Payouts need to be some kind of diminishing return, otherwise you could theoretically earn more from using a part than the original device was worth.

% Assumes they don't change workloads.

% \subsection{Per-Case Measuring}

% % Types of measurements

% The pay-as-you-go model has its benefits, but it also has its technical challenges.


% % Why we are using performance as a proxy for suffering or frustration.

% The first-order and most obvious way to measure the measure the performance cost of a patch is to 

% (systems are not homogeneous
% (benchmark suites not representative of typical user behavior)
% (e.g. most users rarely use FP units)

% Build argument for per-case monitoring and per-case payouts


% % Resale value
% % Liability
% % Pay-as-you-go
% % Flat rate
% % Per-case harm
% % Class action lawsuits

==> takeaways.tex <==
\section{Recommendations}
\label{sec:takeaways}

The data collected by the experiments presented in this work has several uses and interpretations depending on who you are.
We interpret our experiments' results from the point of view of product vendors, regulators and policy makers, and end users.

\subsection{Product Vendors}

% As shown in Experiment \#1, users are not very perceptive to losses of performance when not informed that such losses are taking place.
% Does this mean that despite what users think, performance does not matter to consumers, and that products should be optimized for other features instead?
% Our data shows quite the opposite:
% Even though participants were not very perceptive to changes in performance, they still place a large value on 
% We think it would be a grave mistake to draw this conclusion from our results.
% Instead, we 

Unclear what we should be saying here based on our recent Slack conversations.


\subsection{Regulators and Policy Makers}

Putting a price tag on performance can be a useful datapoint when answering questions of how much companies should have to pay their customers for throttling performance.
As a motivating example, consider the recent class action lawsuits against Apple Inc. for the so-called Batterygate scandal, where Apple was accused of throttling processor performance in older iPhones without users' knowledge or consent\footnote{Apple claims to have done so to improve the reliability and stability of older devices with aging batteries; Its critics contend that the real reason was to incentivize customers into buying newer models of the iPhone.}.
A U.S. District Court ordered Apple to pay a minimum of \$310 million and a maximum of \$500 million to its affected customers as a penalty for for an approximate payout of \$25 per affected customer.
While these class action lawsuits have received the most attention, we point out that similar disputes have yet to be settled, particularly over the performance losses from the Spectre and Meltdown patches.
And in general, we expect that these types of disputes will only become more and more common as hardware and architecture come under increased scrutiny from the research community.

A key question when settling these types disputes is, how much should users be compensated?
If the goal of such lawsuits is to recoup the dollar equivalent of the losses endured by each customer, then the results presented in this work are perfectly designed to help answer these questions.
In particular, Experiment \#2 is especially useful since it prevents participants from reporting unreasonably high WTA prices in an attempt to recoup more money.


\subsection{End Users}

???

==> tasks_table.tex <==
% \begin{table}[]
% \begin{tabular}{|l|c|c|c|c|c|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{}   & \textbf{A}         & \textbf{B}                               & \textbf{C}                              & \textbf{D}                                                                                                                                                                                 & E                                                                                                                                              & \multicolumn{1}{c|}{F}                                                                                                                                                                                        & \multicolumn{1}{c|}{G}           & \multicolumn{1}{c|}{H}                                                                                                & \multicolumn{1}{c|}{I}                                                   \\ \hline
% \textit{\textbf{Task 1}} & Open a web browser & Log in to school-provided internet email & Create a new Google Doc titled "Task 1" & Open Google Maps in a new tab. Find out how long it would take (in hours) to drive from Los Angeles, USA to New York, USA. Write down this number in the previously created Google Doc.    & Open an image search engine in a new tab. Find a photo of Low Library at Columbia University. Copy and paste it into the Google Doc.           & Open YouTube in a new tab. Find a live performance of the classical music piece "Bolero" by composer Maurice Ravel. Copy and paste the video's URL into the Google Doc.                                       & Download the Google Doc as a PDF & Create a new email titled "Task 1". Attach the previously downloaded PDF. Send the email to a provided email address. & Close all tabs and delete the previously created PDF from your computer. \\ \hline
% \textit{\textbf{Task 2}} & Open a web browser & Log in to school-provided internet email & Create a new Google Doc titled "Task 2" & Open Google Maps in a new tab. Find out how long it would take (in hours) to drive from Casablanca, Morocco to Cairo, Egypt. Write down this number in the previously created Google Doc.  & Open an image search engine in a new tab. Find a photo of the Alma Mater statue at Columbia University. Copy and paste it into the Google Doc. & Open YouTube in a new tab. Find a live performance of the classical music piece "Rhapsody in Blue" by composer George Gershwin. Copy and paste the video's URL into the Google Doc.                           & Download the Google Doc as a PDF & Create a new email titled "Task 2". Attach the previously downloaded PDF. Send the email to a provided email address. & Close all tabs and delete the previously created PDF from your computer. \\ \hline
% \textit{\textbf{Task3}}  & Open a web browser & Log in to school-provided internet email & Create a new Google Doc titled "Task 3" & Open Google Maps in a new tab. Find out how long it would take (in hours) to drive from Sydney, Australia to Perth, Australia. Write down this number in the previously created Google Doc & Open an image search engine in a new tab. Find a photo of Butler Library at Columbia University. Copy and paste it into the Google Doc.        & Open YouTube in a new tab. Find a live performance of the classical music piece "Fantasia on a Theme by Thomas Tallis" by composer Ralph Vaughn Williams. Copy and paste the video's URL into the Google Doc. & Download the Google Doc as a PDF & Create a new email titled "Task 3". Attach the previously downloaded PDF. Send the email to a provided email address. & Close all tabs and delete the previously created PDF from your computer. \\ \hline
% \end{tabular}
% \caption{}
% \label{tab:my-table}
% \end{table}

\begin{table}[]
    \begin{tabular}{|p{0.25cm}|p{2.4cm}|p{2.4cm}|p{2.4cm}|}
    \hline
    \textbf{}  & \textbf{Task 1}                                                                                                                                                                         & \textbf{Task 2}                                                                                                                                                                           & \textbf{Task 3}                                                                                                                                                                                               \\ \hline
    \textbf{A} & Open a web browser                                                                                                                                                                      & Open a web browser                                                                                                                                                                        & Open a web browser                                                                                                                                                                                            \\ \hline
    \textbf{B} & Log in to school-provided internet email                                                                                                                                                & Log in to school-provided internet email                                                                                                                                                  & Log in to school-provided internet email                                                                                                                                                                      \\ \hline
    \textbf{C} & Create a new Google Doc titled "Task 1"                                                                                                                                                 & Create a new Google Doc titled "Task 2"                                                                                                                                                   & Create a new Google Doc titled "Task 3"                                                                                                                                                                       \\ \hline
    \textbf{D} & Open Google Maps in a new tab. Find out how long it would take (in hours) to drive from Los Angeles, USA to New York, USA. Write down this number in the previously created Google Doc. & Open Google Maps in a new tab. Find out how long it would take (in hours) to drive from Casablanca, Morocco to Cairo, Egypt. Write down this number in the previously created Google Doc. & Open Google Maps in a new tab. Find out how long it would take (in hours) to drive from Sydney, Australia to Perth, Australia. Write down this number in the previously created Google Doc                    \\ \hline
    \textbf{E} & Open an image search engine in a new tab. Find a photo of Low Library at Columbia University. Copy and paste it into the Google Doc.                                                    & Open an image search engine in a new tab. Find a photo of the Alma Mater statue at Columbia University. Copy and paste it into the Google Doc.                                            & Open an image search engine in a new tab. Find a photo of Butler Library at Columbia University. Copy and paste it into the Google Doc.                                                                       \\ \hline
    \textbf{F} & Open YouTube in a new tab. Find a live performance of the classical music piece "Bolero" by composer Maurice Ravel. Copy and paste the video's URL into the Google Doc.                 & Open YouTube in a new tab. Find a live performance of the classical music piece "Rhapsody in Blue" by composer George Gershwin. Copy and paste the video's URL into the Google Doc.       & Open YouTube in a new tab. Find a live performance of the classical music piece "Fantasia on a Theme by Thomas Tallis" by composer Ralph Vaughn Williams. Copy and paste the video's URL into the Google Doc. \\ \hline
    \textbf{G} & Download the Google Doc as a PDF                                                                                                                                                        & Download the Google Doc as a PDF                                                                                                                                                          & Download the Google Doc as a PDF                                                                                                                                                                              \\ \hline
    \textbf{H} & Create a new email titled "Task 1". Attach the previously downloaded PDF. Send the email to a provided email address.                                                                   & Create a new email titled "Task 2". Attach the previously downloaded PDF. Send the email to a provided email address.                                                                     & Create a new email titled "Task 3". Attach the previously downloaded PDF. Send the email to a provided email address.                                                                                         \\ \hline
    \textbf{I} & Close all tabs and delete the previously created PDF from your computer.                                                                                                                & Close all tabs and delete the previously created PDF from your computer.                                                                                                                  & Close all tabs and delete the previously created PDF from your computer.                                                                                                                                      \\ \hline
    \end{tabular}
    \caption{This table contains a list of the sub-tasks the participants complete at part of Tasks 1, 2 \& 3. (Note: there is a lot of redundant information in this table, but I haven't yet figured out a better way to arrange everything. Any advice is welcome!)}
    \label{tab:my-table}
\end{table}
